Masked Momentum Contrastive Learning for Zero-shot Semantic Understanding

Self-supervised pretraining (SSP) has emerged as a popular technique in machine learning, enabling the extraction of meaningful feature representations without labelled data. In the realm of computer vision, pretrained vision transformers (ViTs) have played a pivotal role in advancing transfer learning. Nonetheless, the escalating cost of finetuning these large models has posed a challenge due to the explosion of model size. This study endeavours to evaluate the effectiveness of pure self-supervised learning (SSL) techniques in computer vision tasks, obviating the need for finetuning, with the intention of emulating human-like capabilities in generalisation and recognition of unseen objects. To this end, we propose an evaluation protocol for zero-shot segmentation based on a prompting patch. Given a point on the target object as a prompt, the algorithm calculates the similarity map between the selected patch and other patches, upon that, a simple thresholding is applied to segment the target. Another evaluation is intra-object and inter-object similarity to gauge discriminatory ability of SSP ViTs. Insights from zero-shot segmentation from prompting and discriminatory abilities of SSP led to the design of a simple SSP approach, termed MMC. This approaches combines Masked image modelling for encouraging similarity of local features, Momentum based self-distillation for transferring semantics from global to local features, and global Contrast for promoting semantics of global features, to enhance discriminative representations of SSP ViTs. Consequently, our proposed method significantly reduces the overlap of intra-object and inter-object similarities, thereby facilitating effective object segmentation within an image. Our experiments reveal that MMC delivers top-tier results in zero-shot semantic segmentation across various datasets.

==> figs/clusters.tex <==

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{pics/pSiT-cluster.png}
    \caption{Cluster visualization for patch features. Patches tokens are split into 10 clusters by K-Means. Models are ViT-B/16 trained on IN1K.}
    \label{fig:feature_maps}
\end{figure}

==> figs/front_segmentation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{pics/instance_retrieval_threshold.png} %
    \caption{zero-shot segmentation. From the left to the right, the figures respectively show the ground-truth segmentation labels, 3 clusters via K-means, similarity distributions, and the predictions for the selected object for threshold.  }
    \label{fig:zero_shot_seg}
\end{figure}

==> figs/global_semantics.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.5\linewidth]{pics/global_semantics.png}
    \caption{Classification performance for CLS token and patch tokens.}
    \label{fig:global_semantic}
\end{figure}

==> figs/similarity_ROC.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.98\linewidth]{pics/similarity_dist/dist_coco.pdf}
    \includegraphics[width=.43\linewidth]{pics/similarity_dist/roc.png}
    \caption{(Left) Similarity Distribution on COCO. (Right) ROC.}
    \label{fig:sim_dist}
\end{figure}

\begin{table}
    \centering
    \caption[short]{Optimal thresholds for separating objects.}\label{tab:threshold}
    \begin{tabular}{lcccccc}
        & \multicolumn{3}{c}{ROC} & \multicolumn{3}{c}{IoU} \\
        model       & threshold & FP$\downarrow$   & TP$\uparrow$   & threshold & FP$\downarrow$   & TP $\uparrow$  \\
        \hline 
        MAE         & 0.53      & 0.28 & 0.53 & 0.14      & 0.93 & 0.97 \\
        iBOT        & 0.27      & 0.27 & 0.63 & 0.17      & 0.55 & 0.83 \\
        DINO        & 0.26      & 0.18 & 0.54 & 0.18      & 0.56 & 0.79 \\
        ours         & 0.82      & 0.19 & 0.57 & 0.75      & 0.52 & 0.81 \\
        ours\_neg    & 0.75      & 0.22 & 0.61 & 0.68      & 0.51 & 0.81 \\
        ours\_iBOT   & 0.65      & 0.23 & 0.66 & 0.58      & 0.43 & 0.81 \\
    \end{tabular}
\end{table}
% import glob,os

% for file in glob.glob('../outputs/pics/similarity/*.pkl.npy'):
%     model_name = os.path.basename(file).split('-')[0]
%     hist_dict = np.load(file,allow_pickle=True)[None][0]
%     inter_density = hist_dict['inter_density']
%     intra_density = hist_dict['intra_density']
    
%     inter_acc = np.cumsum(inter_density)
%     intra_acc = np.cumsum(intra_density)
    
%     acc = (1-intra_acc)/(2-intra_acc-inter_acc)
%     recall = 1 - intra_acc
    
%     # plt.plot(bin_centers, inter_density,label='inter')
%     # plt.plot(bin_centers, intra_density,label="intra")
%     # plt.title(model_name)
%     # break
%     plt.xlabel('recall')
%     plt.ylabel('acc')
%     plt.plot(recall[:-1],acc[:-1],label=model_name)

% plt.xlim(0.9,0.98)
% plt.ylim(0.94,1)
% plt.savefig('../outputs/pics/similarity/metric_zoomin.pdf', pad_inches=0, bbox_inches=None)

==> figs/zero_shot.tex <==
\begin{figure}
    \centering
    % get the mask labels with class-wise ir instance-wise objects.
    % \includegraphics[width=.45\linewidth]{pics/similarity_dist/data_process_sample1.png}%
    % \includegraphics[width=.45\linewidth]{pics/similarity_dist/data_process_sample2.png}
    \includegraphics[width=\linewidth]{pics/similarity_dist/single_point_segment.png}
    \caption{Zero-shot segmentation.}\label{fig:zero_shot}
\end{figure}

==> pics/finetune.tex <==
% \begin{table}[t]
% \centering
% %https://matplotlib.org/stable/gallery/specialty_plots/radar_chart.html
% % https://www.python-graph-gallery.com/391-radar-chart-with-several-individuals
% \caption{\todo{radar chart(aka spider or star chart).}
%         Finetune performance on downstream tasks. w/o denotes the model without multi-crops.}\label{tab:finetune}
% \begin{tabular}{lccccccc}
% % \toprule
%         & Aircraft*       & CIFAR10        & CIFAR100       & Cars           & Flowers        & Pets           & 1N1K\\
% \hline
%  \textit{ViT-S/16 on IN100} &&&&&&\\
% MAE      & 56.59          & 97.87          & 85.04          & 90.14          & 87.49          & 87.65          & -  \\
% MSN      & 74.65          & 97.86          & 84.95          & 87.13          & 87.92          & 86.84          & -  \\
% DINO w/o & 57.31          & 95.69          & 78.33          & 69.58          & 80.31          & 70.07          & -  \\
% DINO     & 69.16          & 97.26          & 83.09          & 84.93          & 87.25          & 82.99          & -  \\
% iBOT w/o & 72.79          & 98.25          & 85.60          & 85.30          & 87.84          & 84.57          & -  \\
% iBOT     & 73.39          & 98.20          & 85.95          & 87.15          & 89.80          & 87.05          & -  \\
% ours w/o & \textbf{79.30} & \textbf{98.41} & \textbf{86.57} & \textbf{90.41} & \textbf{91.90} & \textbf{90.35} & -  \\
%  \midrule
%  \textit{ViT-B/16 on IN1K} &&&&&\\
% iBOT, 1600e     &           & 98.85     & 88.76     & 94.16     & 97.48     & 93.43 & 84.0    \\
% ours w/o, 400e &           & 99.17     & 90.17     & 93.21     & 97.07     & 94.11 & 83.0 \\
% ours (c=10) \\
% % \bottomrule
% \end{tabular}

% \end{table}



==> tabs/classification_IN1K.tex <==
% classification performance comparison for fine-tuning models pre-trained on IN1K.
\begin{table*}[]
    \centering
    \begin{tabular}{@{}ll|cccccc@{}}
    \toprule
    Method                           & Epoch & Flwrs         & Pets          & Cars          & C10           & C100          & IN1K          \\ 
    % \cmidrule(r){3-8}
    \midrule
    MoCo-v3 \cite{chen_empirical_2021} & 300   & 98.3          & 93.7          & 93.4          & 98.2          & 87.3          & 83.2          \\
    Dino \cite{caron_emerging_2021}    & 400   & 98.4          & 90.2          & 93.0          & 98.2          & 87.1          & 82.8          \\
    SimMIM \cite{xie_simmim_2022}  &  800  & 97.2          & 92.3          & 91.5          & 98.9          & 88.6          & 83.6          \\
    MAE \cite{he_masked_2022}     & 1600  & 98.9          & 92.8          & 93.5          & 99.0          & --            & 83.4          \\
    iBOT \cite{zhou_ibot_2022}    & 1600  & \textbf{97.5} & 93.4          & \textbf{94.2} & 98.9          & 88.8          & \textbf{84.0} \\
    MMC                             & 800   & 97.1          & \textbf{94.1} & 93.2          & \textbf{99.2} & \textbf{90.2} & 83.5          \\ 
    \bottomrule
    \end{tabular}
    \captionof{table}{Transfer learning by finetuning models pretrained on ImageNet-1K dataset accross various downstream datasets. We report top-1 accuracy.}
    \label{tab:large_scale_classification}
\end{table*}

==> tabs/knn.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{wraptable}{r}{6.2cm}
\captionsetup{width=.95\linewidth}
\caption{KNN classification of ViTs on four datasets using three types of projections. 
% The table shows top-1 accuracy (\%) pretrained on IN1K. Note that the accuracy values for the MAE are based on normalized features along the batch.
% The three types of heads used for classification are: the CLS token (0), the mean of patch tokens (1), the concatenation of the above (2).
}\label{tab:KNN1K}
\centering
\setlength{\tabcolsep}{0.76mm}{
\begin{tabular}{lcccc}

Dataset    & IN100    & CIFAR10        & Flowers        & Pets           \\ 
\toprule
\multicolumn{5}{c}{CLS token}                              \\  
ours \rule{0pt}{3ex}  & 89.94          & \textbf{96.37} & 78.16          & \textbf{89.94} \\
DINO & 91.54          & 96.07          & 85.75          & 90.38          \\
iBOT & \textbf{92.12} & 96.15          & \textbf{84.47} & 89.10          \\ \midrule 
\multicolumn{5}{c}{Patch tokens}            \\  
ours \rule{0pt}{3ex}   & \textbf{90.04} & \textbf{96.67} & \textbf{74.43} & \textbf{90.22} \\
DINO & 75.56          & 87.25          & 71.61          & 70.81          \\
iBOT & 75.22          & 90.38          & 64.76          & 49.74          \\
MAE*  & 70.88          & 76.53          & 66.32          & 53.64          \\ \midrule 
ours      &                \multicolumn{4}{c}{Hyber tokens}    \\  
0          & 89.94          & 96.37          & \textbf{78.16} & 89.94          \\
1          & 90.04          & \textbf{96.67} & 74.43          & 90.22          \\
2          & \textbf{90.48} & 96.51          & 77.20          & \textbf{90.35} \\ 

\end{tabular}
}
\end{wraptable}



% \begin{table*}[]
% \centering
% \begin{tabular}{lcccccc}
% \toprule
%          & Aircraft       & CIFAR10        & CIFAR100       & Cars  & Flowers        & Pets           \\
%  \midrule
% mae-500  & 8.40           & 49.94          & 22.16          & 4.20           & 21.22 &  11.64          \\
% msn      & 20.25          & 77.76          & 52.42          & 11.98          & 57.80 &  55.44          \\ 
% dino (w/o)  & 17.94       & 76.35          & 51.35          & 13.22       & 57.62  & 38.29          \\
% dino-500 & \textbf{21.99} & 76.64          & 53.33          & \textbf{18.02} & \textbf{67.59} & 52.71          \\
% ibot-wo  & 14.94          & 68.18          & 43.21          & 11.07          & 57.02 &  43.15          \\
% ibot-500 & 15.54          & 68.89          & 45.15          & 14.13          & 61.26 &  47.10          \\
% cssl-500 & 21.75          & \textbf{84.86} & \textbf{62.17} & 14.40          & 65.49 &  \textbf{62.44} \\
% \bottomrule
% \end{tabular}
% \caption{$k$-NN classification on downstream tasks. DINO (w/o) and iBOT (w/o) remove multi-crops augmentation during pretraining.}\label{tab:KNN}
% \end{table*}

==> tabs/knn_setting.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\caption{$k$-NN for the number of neighbours (K) and the types of projection.}
\label{tab:knn_setting}
\begin{tabular}{lcccc|cccc|cccc}
Projection &   \multicolumn{4}{c}{CLS token}              & \multicolumn{4}{c}{Patch tokens}              & \multicolumn{4}{c}{Hyber tokens}     \\ 
Data/K      & 10            & 20   & 50   & 100  & 10            & 20   & 50   & 100  & 10   & 20   & 50   & 100  \\
\hline
Cars        & \textbf{14.5} & 13.9 & 12.8 & 12.3 & 13.8          & 13.4 & 12.5 & 12.2 & 14.4 & 13.4 & 12.5 & 11.9 \\
Flowers     & 63.5          & 59.6 & 54.8 & 52.9 & \textbf{66.0} & 63.8 & 62.0 & 61.1 & 65.5 & 62.5 & 59.4 & 58.2 \\
CIFAR10    & 84.5          & 83.9 & 82.7 & 80.9 & \textbf{84.9} & 84.5 & 83.3 & 82.0 & 84.8 & 84.6 & 83.0 & 81.8 \\ 

\end{tabular}
\end{table*}

==> tabs/linprob.tex <==
\begin{table*}[]
\centering
\caption{Linear prob on downstream tasks. w/o denotes the model without multi-crops.}\label{tab:linprob}
\begin{tabular}{@{}llcccccc@{}}
% \toprule
 Arch.    & \textbf{}  & Aircraft & CIFAR10        & CIFAR100       & Cars           & Flowers & Pets           \\ 
\midrule
 ViT-S/16%
 & MAE  & 18.33          & 64.66          & 43.95          & 13.29          & 52.89          & 32.73          \\
 & MSN      & 36.57          & 59.27          & 63.11          & 41.04          & 82.22          & 75.03          \\
 & DINO-w/o  & 29.88          & 76.85          & 57.42          & 26.58          & 72.92          & 54.73          \\
 & DINO & 40.11          & 80.00          & 62.21          & 39.60          & 80.50          & 68.22          \\
 & iBOT-w/o  & 29.64          & 74.92          & 54.82          & 29.19          & 77.95          & 67.54          \\
 & iBOT & 32.46          & 74.74          & 55.69          & 31.49          & 80.03          & 66.78          \\
 & ours & \textbf{43.44} & \textbf{87.81} & \textbf{71.38} & \textbf{45.39} & \textbf{84.03} & \textbf{82.77} \\
\midrule      
{\color[HTML]{9B9B9B} ResNet50} & {\color[HTML]{9B9B9B} Supervised} & {\color[HTML]{9B9B9B} 36.78}    & {\color[HTML]{9B9B9B} 86.16}    & {\color[HTML]{9B9B9B} 62.70}    & {\color[HTML]{9B9B9B} 30.61}    & {\color[HTML]{9B9B9B} 76.09}    & {\color[HTML]{9B9B9B} 73.50}    \\
{\color[HTML]{9B9B9B} }         & {\color[HTML]{9B9B9B} LoGo}       & {\color[HTML]{9B9B9B} 50.07}    & {\color[HTML]{9B9B9B} 86.09}    & {\color[HTML]{9B9B9B} 63.43}    & {\color[HTML]{9B9B9B} 40.77}    & {\color[HTML]{9B9B9B} 92.13}    & {\color[HTML]{9B9B9B} 76.17}    \\
                     
\end{tabular}

\end{table*}

==> tabs/recipes.tex <==

\begin{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% mini page table 1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[t]{\linewidth}
    \begin{tabular}{l|l} 
    config & IN1K \\
    \hline optimizer & AdamW \\
    base learning rate & 0.001 \\
    weight decay & 0 \\
    optimizer momentum & 0.9 \\
    batch size & 16384 \\
    learning rate schedule & cosine decay \\
    warmup epochs & 10 \\
    training epochs & 90 \\
    augmentation & RandomResizedCrop
    \end{tabular}
    \caption{Linprob recipe.}
    \label{tab:setting_linprob}
\end{minipage}%

\begin{minipage}[t]{\linewidth}

    \begin{tabular}{l|l} 
    config & IN1K \\
    \hline optimizer & AdamW \\
    base learning rate & 0.001 \\
    weight decay & 0.05 \\
    optimizer momentum & 0.9 \\
    batch size & 256 \\
    learning rate schedule & cosine decay \\
    warmup epochs & 10 \\
    training epochs & 90 \\
    augmentation & RandAug
    \end{tabular}
    \caption{Finetune recipe.}
    \label{tab:setting_finetune}
\end{minipage}
\end{table}

==> tabs/rep_stability.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

